Towards Controlled Table-to-Text Generation with Scientific Reasoning

The sheer volume of scientific experimental results and complex technical statements, often presented in tabular formats, presents a formidable barrier to individuals acquiring preferred information. The realms of scientific reasoning and content generation that adhere to user preferences encounter distinct challenges. In this work, we present a new task for generating fluent and logical descriptions that match user preferences over scientific tabular data, aiming to automate scientific document analysis. To facilitate research in this direction, we construct a new challenging dataset CTRLSciTab consisting of table-description pairs extracted from the scientific literature, with highlighted cells and corresponding domain-specific knowledge base. We evaluated popular pre-trained language models to establish a baseline and proposed a novel architecture outperforming competing approaches. The results showed that large models struggle to produce accurate content that aligns with user preferences. As the first of its kind, our work should motivate further research in scientific domains.

==> Files/related_work.tex <==
\section{Related Work}

\subsection{Table-to-text Generation}
The traditional task of table-to-text generation is to generate coherent descriptions based on tabular data. To meet this requirement, several data sets have been developed, such as WikiBio \cite{liu2018table}, WikiTableT \cite{chen2021wikitablet}, ToTTo \cite{RN115}, and LogicNLG \cite{RN153}. These data sets focus primarily on general domains and are taken from Wikipedia. There has recently been a growing need for reasoning-aware generation, which has led to a surge of interest in advanced table-to-text generation incorporating numerical reasoning. To facilitate research in this area, several data sets have been proposed, including RotoWire \cite{wiseman2017challenges}, SportSett \cite{thomson2020sportsett}, numericNLG \cite{suadaa2021towards}, and SciGen \cite{moosavi2021scigen}. \newline

However, the impressive performance of large PLMs such as GPT4 \cite{OpenAI2023GPT4TR} and Llama \cite{touvron2023llama} has led to a shift in research requirements from generic generation to more specific areas that necessitate domain-specific knowledge. In contrast to the previous table-to-text generation task, we propose a new research problem focused on controlled table-to-text generation with common sense reasoning. Given that tabular data align with domain-specific knowledge, the system is required to produce satisfactory text outputs. This research problem explicitly tests the ability of machines to generate analytical descriptions that are consistent with domain-specific common sense while satisfying user preferences. To advance research in this direction, we present a novel challenging data set, CTRLSciTab, which consists of table-description pairs extracted from the scientific literature. This data set contains highlighted cells representing user preferences and corresponding domain-specific knowledge for common sense reasoning.

\subsection{NLG with Common Sense Reasoning}
Generating fluent descriptions that incorporate common sense reasoning presents a challenge to PLMs' reading comprehension abilities. While previous studies have primarily focused on language generation with practical knowledge and experience of open domains \cite{lin2020commongen}, these studies have explored various aspects of language generation, including entity extraction \cite{xu2018automatic}, \cite{li2016commonsense}, question answering \cite{talmor2019commonsenseqa}, \cite{huang2019cosmos}, \cite{wang2019does}, and cultural and social analysis \cite{lin2018mining}, \cite{sap2019atomic}. Additionally, downstream applications such as image captioning \cite{lu2018neural}, video storytelling \cite{yang2019knowledgeable}, and conversational systems \cite{zhang2020grounded} have demonstrated great potential for common sense reasoning. In contrast to previous studies, we propose the first task of table-to-text generation with common sense reasoning to the best of our knowledge. To support research in this direction, we introduce a new data set, CTRLSciTab, which consists of scientific tabular data that adheres to domain-specific knowledge.




